A proof theory of right-linear (omega-)grammars via cyclic proofs

Right-linear (or left-linear) grammars are a well-known class of context-free grammars computing just the regular languages. They may naturally be written as expressions with (least) fixed points but with products restricted to letters as left arguments, giving an alternative to the syntax of regular expressions. In this work, we investigate the resulting logical theory of this syntax. Namely, we propose a theory of right-linear algebras (RLA) over of this syntax and a cyclic proof system CRLA for reasoning about them. We show that CRLA is sound and complete for the intended model of regular languages. From here we recover the same completeness result for RLA by extracting inductive invariants from cyclic proofs, rendering the model of regular languages the free right-linear algebra. Finally, we extend system CRLA by greatest fixed points, nuCRLA, naturally modelled by languages of omega-words thanks to right-linearity. We show a similar soundness and completeness result of (the guarded fragment of) nuCRLA for the model of omega-regular languages, employing game theoretic techniques.

==> bootstrapping.tex <==
% \section{Bootstrapping $\RLA$: canonical systems and meets}

% \subsection{Functoriality}

% \begin{lemma}[Functoriality]
% \label{lemma:RLA-functoriality}
% If $\RLA \proves f \leq g$ then $\RLA\proves e[f/X] \leq e[g/X]$
% \end{lemma}

% \begin{proof}
% By induction on $e$. For the induction to go through, we will prove a stronger statement \textit{viz.} if $\RLA\proves (f_i\leq g_i)_{i\in[n]}$, then $\RLA\proves e[f_1/X_1,\dots,f_n/X_n]\leq e[g_1/X_1,\dots,g_n/X_n]$.

% \begin{itemize}
%     \item It is vacuously true if none of the $X_i$s occurs freely in $e$. If $e=X_i$ for some $i$, it is identity.
%     \item If $e=f+g$ or $e=af$, then we have easy induction cases.
%     \item If $e=\mu Yf$, we have the following where $h=\mu Yf[\overline g/\overline X]$ and $\overline f/\overline X$ and $\overline g/\overline X$ denotes $f_1/x_1,\dots,f_n/x_n$ and $g_1/x_1,\dots,g_n/x_n$ respectively.

%     Since $h\leq h$, we get by induction hypothesis, that $f[h/Y,\overline f/\overline X]\leq f[h/Y,\overline g/\overline X]$. But $f[h/Y,\overline g/\overline X]\leq h$ and so, $f[h/Y,\overline f/\overline X]\leq h$. Therefore, $\mu Y.f[\overline f/\overline X]\leq h$.
% \end{itemize}
% \end{proof}



